Exploring the Interplay Between Colorectal Cancer Subtypes Genomic Variants and Cellular Morphology: A Deep-Learning Approach

Molecular subtypes of colorectal cancer (CRC) significantly influence treatment decisions. While convolutional neural networks (CNNs) have recently been introduced for automated CRC subtype identification using H&E stained histopathological images, the correlation between CRC subtype genomic variants and their corresponding cellular morphology expressed by their imaging phenotypes is yet to be fully explored. The goal of this study was to determine such correlations by incorporating genomic variants in CNN models for CRC subtype classification from H&E images. We utilized the publicly available TCGA-CRC-DX dataset, which comprises whole slide images from 360 CRC-diagnosed patients (260 for training and 100 for testing). This dataset also provides information on CRC subtype classifications and genomic variations. We trained CNN models for CRC subtype classification that account for potential correlation between genomic variations within CRC subtypes and their corresponding cellular morphology patterns. We assessed the interplay between CRC subtypes' genomic variations and cellular morphology patterns by evaluating the CRC subtype classification accuracy of the different models in a stratified 5-fold cross-validation experimental setup using the area under the ROC curve (AUROC) and average precision (AP) as the performance metrics. Combining the CNN models account for variations in CIMP and SNP further improved classification accuracy (AUROC: 0.847$\pm$0.01 vs. 0.787$\pm$0.03, p$=$0.01, AP: 0.68$\pm$0.02 vs. 0.64$\pm$0.05).

==> figures/data_split.tex <==

%\documentclass[border=15pt, multi, tikz]{standalone}
%\usepackage{import}
%\usetikzlibrary{positioning,matrix}
%\usetikzlibrary{shapes}
%\usetikzlibrary{plotmarks}
%\usetikzlibrary{decorations.pathreplacing,calligraphy}
%\begin{document}
\begin{adjustbox}{width=\linewidth}  
\begin{tikzpicture}[font=\normalsize,thick]
% Start block
\node[draw,
    minimum width=2.5cm,
    minimum height=1cm] (block2) {Entire Cohort - n=430};
    

% Power and voltage variation
\node[draw,
    align=center,
    below=of block2,
    minimum width=3.5cm,
    minimum height=1cm
] (block3) {Pre-processed by Kather et al. - n=360};


% Conditions test
\node[draw,
    align=center,
    circle,
    below right=of block3,
    minimum width=2.5cm,
    text width=2cm,
    inner sep=0,fill=red!30] (block4) {Test - n=100, p=98,904};
    
\node[draw,
    align=center,
    circle,
    below left=of block3,
    minimum width=2.5cm,
    text width=2cm,
    inner sep=0,fill=red!30] (block5) {Train - n=260, p=93,408};
   


\node[draw=black,
    below left=of block4,
    minimum width=2.5cm,
    text width=2.5cm,
    minimum height=1cm, fill=green!30] (block6) 
    { MSI: \\ n=26, p=28,335};
    

\node[draw=black,
    below right=of block4,
    minimum width=2.5cm,
    text width=2.7cm,
    minimum height=1cm,fill=green!30] (block7) 
    { MSS: \\ n=74, p=70,569};
   

    
\node[draw=black,
    below left=of block5,
    minimum width=2.5cm,
    text width=2.5cm,
    minimum height=1cm, fill=green!30] (block8) 
    { MSI: \\ n=39, p=46,704};
    


\node[draw=black,
    below right=of block5,
    minimum width=2.5cm,
    text width=2.5cm,
    minimum height=1cm,fill=green!30] (block9)  { MSS: \\ n=221, p=46,704};


    
% Arrows
\draw[-latex] 
    (block2) edge (block3)
    (block3) edge (block4);

\draw[-latex] (block3) -- (block5)
    node[pos=0.25,fill=white,inner sep=0]{};
\draw[-latex] (block4) -| (block6)
 node[pos=0.25,fill=white,inner sep=0]{};
    
\draw[-latex] (block4) -| (block7)
    node[pos=0.25,fill=white,inner sep=0]{};
\draw[-latex] (block5) -| (block8)
 node[pos=0.25,fill=white,inner sep=0]{};
    
\draw[-latex] (block5) -| (block9)
    node[pos=0.25,fill=white,inner sep=0]{};
    




\end{tikzpicture}

\end{adjustbox}
%\end{document}

==> figures/flow.tex <==
   \begin{adjustbox}{width=\linewidth}  
\begin{tikzpicture}[font=\normalsize,thick]
% Start block
\node[draw,
    %minimum width=2.5cm,
    minimum height=1cm] (kather) {TCGA-CRC-DX - n=360};

\node[draw,
    %minimum width=2.5cm,
    right of = kather,
    minimum height=1cm] (baseline) {Baseline model};

\node[draw,
    %minimum width=2.5cm,
    right of = baseline,
    minimum height=1cm] (molecular) {Molecular feature analysis};
\begin{comment}
\node[draw,
    minimum width=2.5cm,
    right of = molecular,
    minimum height=1cm] (BP-classes) {BP classes};

\node[draw,
    minimum width=2.5cm,
     below right of = BP-classes,
    minimum height=1cm] (SNP) {BP-CNN\textsubscript{SNP}};

\node[draw,
    minimum width=2.5cm,
    below left of = BP-classes,
    minimum height=1cm] (CIMP) {BP-CNN\textsubscript{CIMP}};

\node[draw,
    minimum width=2.5cm,
    below left of = SNP,
    minimum height=1cm] (Combined) {BP-CNN\textsubscript{Combined}};
\end{comment}
        
% Arrows
\draw[-latex] 
    (kather) edge (baseline);
\draw[->](baseline) -- (molecular);
%\draw[-latex](molecular) edge (BP-classes);
%\draw[-latex](BP-classes) edge (SNP);
%\draw[-latex](BP-classes) edge (CIMP);
%\draw[-latex](SNP) edge (Combined);
%\draw[-latex](CIMP) edge (Combined);

    


\end{tikzpicture}

\end{adjustbox}

==> figures/patient-agg.tex <==
\usetikzlibrary{positioning,matrix, arrows.meta}
\usetikzlibrary{shapes,arrows}

\tikzstyle{block} = [draw, rectangle, 
    minimum height=3em, minimum width=6em,fill=blue!30]
\tikzstyle{circ} = [draw, circle, node distance=1cm,fill=red!30]
\tikzstyle{input} = [coordinate]
\begin{tikzpicture}
\node [input, name=input] {};
\node [block] (inception) at (0,0) {Feature extractor};
\node [block] (mlp) at (3,0) {classifier};
\node(D) at(1,3) {Patch level};
\node [circ, above right=of mlp] (msi) {MSI};
\node(C) [above=0.4cm of msi]{Softmax};
\node [circ, below right=of mlp] (mss) {MSS};
\matrix (A) [matrix of nodes, right=2cm of msi, nodes={draw, minimum size=8mm},column sep=-\pgflinewidth]
{    $p_1$\\$p_2$\\\vdots\\$p_N$\\};
\node(B)[right=of A]{
    \(P_w(MSI) = \frac{\sum_{i=1}^{N}p_i(MSI)}{N}\)};
\node(C) [above=of B]{Patient aggregation};
\draw [->] (inception.east) -- (mlp.west);
\draw [->] (mlp.east) -- (msi.west);
\draw [->] (mlp.east) -- (mss.west);
\draw [->] (msi.east) -- (A.west);
\draw[->] (A.east) -- (B.west);
\end{tikzpicture}


==> figures/sub_label_agg.tex <==
\usetikzlibrary{positioning,matrix, arrows.meta}
\usetikzlibrary{shapes,arrows}

\tikzstyle{block} = [draw, rectangle, 
    minimum height=3em, minimum width=6em,fill=blue!30]
\tikzstyle{circ} = [draw, circle, node distance=1cm,fill=red!30]
\tikzstyle{input} = [coordinate]
\begin{tikzpicture}
\node [input, name=input] {};
\node [block] (inception) at (0,0) {Feature extractor};
\node [block] (mlp) at (3,0) {classifier};
\node(D) at(1,3) {Patch level};
\node [circ, above right=of mlp] (msi1) {$MSI_1$};
\node(C) [above=0.4cm of msi]{Softmax};
\node [circ, below right=of mlp] (mss) {MSS};
\node [circ, right=0.4cm of mlp] (msi2) {$MSI_2$};
\matrix (A) [matrix of nodes, right=3cm of msi1, nodes={draw, minimum size=8mm},
    column sep=-\pgflinewidth]{
    $p_1$\\$p_2$\\\vdots\\$p_N$\\};
\node(B)[right=of A]{
    \(P_w(MSI) = \frac{\sum_{i=1}^{N}p_i(MSI)}{N}\)};
\node(C) [above=of B]{Patient aggregation};
\draw [->] (inception.east) -- (mlp.west);
\draw [->] (mlp.east) -- (msi1.west);
\draw [->] (mlp.east) -- (msi2.west);
\draw [->] (6.5,1) -- (8.5,1) node[midway,above]{max($MSI_1$,$MSI_2$)};
\draw [->] (mlp.east) -- (mss.west);
\draw[->] (A.east) -- (B.west);
\end{tikzpicture}

